Tackling Climate Change with Machine Learning

Climate change is one of the greatest challenges facing humanity, and we, as machine learning experts, may wonder how we can help. Here we describe how machine learning can be a powerful tool in reducing greenhouse gas emissions and helping society adapt to a changing climate. From smart grids to disaster management, we identify high impact problems where existing gaps can be filled by machine learning, in collaboration with other fields. Our recommendations encompass exciting research questions as well as promising business opportunities. We call on the machine learning community to join the global effort against climate change.

==> AI + Climate Change/figures/end_table.tex <==
\begin{table}
\begin{small}
\begin{center}
\begin{tabular}{l l l l l l l l l l }  \toprule
     \multicolumn{2}{l}{ }
         & \small{\rotatebox{90}{\parbox{2.4cm}{Accelerated\\experimentation}}}
         & \small{\rotatebox{90}{\parbox{2.4cm}{Control systems}}}
         & \small{\rotatebox{90}{\parbox{2.4cm}{Forecasting}}}
         & \small{\rotatebox{90}{\parbox{2.4cm}{Human\\interaction}}}
         & \small{\rotatebox{90}{\parbox{2.4cm}{Hybrid physical\\models}}}
         & \small{\rotatebox{90}{\parbox{2.4cm}{Predictive\\maintenance}}}
         & \small{\rotatebox{90}{\parbox{2.4cm}{Remote sensing}}}
         & \small{\rotatebox{90}{\parbox{2.4cm}{System\\optimization}}}
 %        & \small{\rotatebox{90}{\parbox{2.7cm}{Human interaction}}}
    \\ \midrule
    \rowcolor{ccai-yellow}
    \multicolumn{2}{l}{1 \hyperref[sec:electricity-systems]{Electricity systems}} 
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         &\\ %System optimization
    & \hyperref[sec:electricity-lowCarbon]{Enabling low-carbon electricity}
         & $\bullet$%Accelerated\\experimentation
         & $\bullet$%Control systems
         & $\bullet$%Forecasting
         &
         & $\bullet$%Hybrid physical\\models
         & $\bullet$%Predictive\\maintenance}         
         & $\bullet$%Remote sensing
         & $\bullet$\\%System optimization
    & \hyperref[sec:electricity-currentSystemImpact]{Reducing current-system impacts}
         & %Accelerated\\experimentation
         & %Control systems
         & $\bullet$%Forecasting
         &
         & %Hybrid physical\\models
         & $\bullet$%Predictive\\maintenance}         
         & $\bullet$%Remote sensing
         & \\%System optimization
    & \hyperref[sec:electricity-developing]{Ensuring global impact}
         & %Accelerated\\experimentation
         & %Control systems
         & $\bullet$%Forecasting
         &
         & $\bullet$%Hybrid physical\\models
         & %Predictive\\maintenance}         
         & $\bullet$%Remote sensing
         & \\%System optimization
    \rowcolor{ccai-yellow}
    \multicolumn{2}{l}{2 \hyperref[sec:transportation]{Transportation}} 
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    & \hyperref[sec:TReducing]{Reducing transport activity}
         & $\bullet$%Accelerated\\experimentation
         & $\bullet$%Control systems
         & $\bullet$%Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & $\bullet$%Remote sensing
         & $\bullet$\\%System optimization
   & \hyperref[sec:TEfficient]{Improving vehicle efficiency}
         & $\bullet$%Accelerated\\experimentation
         & $\bullet$%Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & $\bullet$ \\ %System optimization
   & \hyperref[sec:TFuels]{Alternative fuels \& electrification}
         & $\bullet$%Accelerated\\experimentation
         & $\bullet$%Control systems
         & $\bullet$%Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         &$\bullet$\\ %System optimization
   & \hyperref[sec:modalshift]{Modal shift}
         & %Accelerated\\experimentation
         & $\bullet$%Control systems
         & $\bullet$%Forecasting
         & $\bullet$ % human
         & %Hybrid physical\\models
         & $\bullet$%Predictive\\maintenance}         
         & $\bullet$%Remote sensing
         & $\bullet$\\ %System optimization
    \rowcolor{ccai-yellow}
    \multicolumn{2}{l}{3 \hyperref[sec:buildings-cities]{Buildings and cities}} 
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         &  %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         &\\ %System optimization
    & \hyperref[sec:indv]{Optimizing buildings}
         & %Accelerated\\experimentation
         & $\bullet$%Control systems
         & $\bullet$%Forecasting
         &
         & $\bullet$%Hybrid physical\\models
         & $\bullet$%Predictive\\maintenance}         
         & %Remote sensing
         &$\bullet$\\ %System optimization
    & \hyperref[sec:distr]{Urban planning}
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & $\bullet$%Remote sensing
         &\\ %System optimization
    & \hyperref[sec:cities]{The future of cities}
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         &$\bullet$\\ %System optimization
    \rowcolor{ccai-yellow}
    \multicolumn{2}{l}{4 \hyperref[sec:industry]{Industry}} 
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         &\\ %System optimization
    & \hyperref[sec:supplychains]{Optimizing supply chains}
         & %Accelerated\\experimentation
         & $\bullet$%Control systems
         &$\bullet$ %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         &$\bullet$\\ %System optimization
    & \hyperref[sec:materialsandconstruction]{Improving materials}
         & $\bullet$%Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         &\\ %System optimization
    & \hyperref[sec:demandresponse]{Production \& energy}
         & %Accelerated\\experimentation
         & $\bullet$%Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & $\bullet$%Predictive\\maintenance}         
         & %Remote sensing
         &$\bullet$\\ %System optimization
    \rowcolor{ccai-yellow}
    \multicolumn{2}{l}{5 \hyperref[sec:afolu]{Farms \& forests}} 
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         &%Remote sensing
         &\\ %System optimization
    & \hyperref[sec:emissions-detection]{Remote sensing of emissions}
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         &$\bullet$ %Remote sensing
         &\\ %System optimization
    & \hyperref[sec:agriculture]{Precision agriculture}
         & %Accelerated\\experimentation
         & $\bullet$%Control systems
         & $\bullet$%Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & $\bullet$%Remote sensing
         &\\ %System optimization
    & \hyperref[sec:peatlands]{Monitoring peatlands}
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         &$\bullet$ %Remote sensing
         &\\ %System optimization
    & \hyperref[sec:forests]{Managing forests}
         & %Accelerated\\experimentation
         & $\bullet$%Control systems
         & $\bullet$%Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         &$\bullet$ %Remote sensing
         &\\ %System optimization
    \rowcolor{ccai-yellow}
    \multicolumn{2}{l}{6 \hyperref[sec:ccs]{Carbon dioxide removal}}
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         &\\ %System optimization
    & \hyperref[sec:ccs]{Direct air capture}
         & $\bullet$%Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & $\bullet$%Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         &\\ %System optimization
    & \hyperref[subsubsec: sequestrativervin]{Sequestering~\cd}
         & %Accelerated\\experimentation
         &%Control systems
         & %Forecasting
         &
         & $\bullet$%Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    \rowcolor{ccai-yellow}\multicolumn{2}{l}{7 \hyperref[sec: climate prediction]{Climate prediction}}
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    & \hyperref[sec:climate-models-params]{Uniting data, ML \& climate science}
         & %Accelerated\\experimentation
         & %Control systems
         & $\bullet$%Forecasting
         &
         & $\bullet$%Hybrid physical\\models
         & %Predictive\\maintenance}         
         & $\bullet$%Remote sensing
         & \\%System optimization
    & \hyperref[sec:models-extreme-events]{Forecasting extreme events}
         & %Accelerated\\experimentation
         & %Control systems
         &$\bullet$ %Forecasting
         &
         & $\bullet$%Hybrid physical\\models
         & %Predictive\\maintenance}         
         & $\bullet$%Remote sensing
         & \\%System optimization
    \rowcolor{ccai-yellow}
    \multicolumn{2}{l}{8 \hyperref[sec:societal-impacts]{Societal impacts}} 
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         &\\ %System optimization
    & \hyperref[subsub:ecology]{Ecology}
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & $\bullet$%Remote sensing
         &\\ %System optimization
    & \hyperref[subsub:infrastructure]{Infrastructure}
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & $\bullet$%Predictive\\maintenance}         
         & %Remote sensing
         &$\bullet$\\ %System optimization
    & \hyperref[subsub:social_systems]{Social systems}
         & %Accelerated\\experimentation
         & %Control systems
         & $\bullet$%Forecasting
         & $\bullet$
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & $\bullet$%Remote sensing
         & $\bullet$\\%System optimization
    & \hyperref[subsub:crisis]{Crisis}
         & %Accelerated\\experimentation
         & %Control systems
         & $\bullet$%Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & $\bullet$%Remote sensing
         & \\%System optimization
    \rowcolor{ccai-yellow}
    \multicolumn{2}{l}{9 \hyperref[sec:geoengineering]{Solar geoengineering}} 
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    & \hyperref[subsub:better-aerosols]{Understanding \& improving aerosols}
         & %Accelerated\\experimentation
         & $\bullet$%Control systems
         & %Forecasting
         &
         & $\bullet$%Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    & \hyperref[subsub:planetary-control]{Engineering a planetary control system}
         & %Accelerated\\experimentation
         & $\bullet$%Control systems
         & %Forecasting
         &
         & $\bullet$%Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    & \hyperref[subsub:impact-models]{Modeling impacts}
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         &
         & $\bullet$%Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    \rowcolor{ccai-yellow}
    \multicolumn{2}{l}{10 \hyperref[sec:tools-individuals]{Individual action}} 
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         & 
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    & \hyperref[sec:personal_carbon_footprint]{Understanding personal footprint}
         & %Accelerated\\experimentation
         & %Control systems
         & $\bullet$%Forecasting
         & $\bullet$
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    & \hyperref[sec:behavior_change]{Facilitating behavior change}
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         & $\bullet$
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    \rowcolor{ccai-yellow}
    \multicolumn{2}{l}{11 \hyperref[sec:toolsforsociety]{Collective decisions}} 
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         & 
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    & \hyperref[sec:coordination]{Modeling social interactions}
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         & $\bullet$
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    & \hyperref[sec:decisionmaking]{Informing policy}
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         & $\bullet$
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    & \hyperref[subsec:markets]{Designing markets}
         & %Accelerated\\experimentation
         & %Control systems
         & $\bullet$%Forecasting
         &
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & $\bullet$\\%System optimization
    \rowcolor{ccai-yellow}
    \multicolumn{2}{l}{12 \hyperref[sec:education]{Education}} 
         & %Accelerated\\experimentation
         & %Control systems
         & %Forecasting
         & $\bullet$
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    \rowcolor{ccai-yellow}
    \multicolumn{2}{l}{13 \hyperref[sec:finance]{Finance}} 
         & %Accelerated\\experimentation
         & %Control systems
         & $\bullet$%Forecasting
         & $\bullet$
         & %Hybrid physical\\models
         & %Predictive\\maintenance}         
         & %Remote sensing
         & \\%System optimization
    \bottomrule
\end{tabular}
\caption{Cross-cutting objectives that are relevant to many climate change domains.}
\label{tab:themes}
\end{center}
\end{small}
\end{table}


==> AI + Climate Change/figures/intro_table.tex <==
\begin{table}
\begin{small}
\begin{center}
\begin{tabular}{l l l l l l l l l l l l}  \toprule
     \multicolumn{2}{l}{ }
         & \small{\rotatebox{90}{\parbox{2.2cm}{Causal\\inference}}}
         & \small{\rotatebox{90}{\parbox{2.2cm}{Computer\\vision}}}
         & \small{\rotatebox{90}{\parbox{2.2cm}{Interpretable\\models}}}
         & \small{\rotatebox{90}{NLP}}
         & \small{\rotatebox{90}{\parbox{2.2cm}{RL \& Control}}}
        %  & \small{\rotatebox{90}{Robotics}}
         & \small{\rotatebox{90}{\parbox{2.2cm}{Time-series analysis}}}
         & \small{\rotatebox{90}{\parbox{2.2cm}{Transfer\\learning}}}
         & \small{\rotatebox{90}{\parbox{2.2cm}{Uncertainty\\quantification}}}
         & \small{\rotatebox{90}{\parbox{2.2cm}{Unsupervised\\learning}}}
    \\ \midrule
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{1 \hyperref[sec:electricity-systems]{Electricity systems}} 
        & % Causal inf
        &  % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised \ref{sub
    & \hyperref[sec:electricity-lowCarbon]{Enabling low-carbon electricity}
        & % Causal inf
        & $\bullet$% Comp vision
        & $\bullet$% % Interpretable ml
        & % % nlp
        & $\bullet$%% rl + control
        & $\bullet$% % time series
        & % transfer
        & $\bullet$% % UQ
        & $\bullet$\\% unsupervised 
    & \hyperref[sec:electricity-currentSystemImpact]{Reducing current-system impacts}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & $\bullet$% % time series
        & % transfer
        & $\bullet$% % UQ
        & $\bullet$\\% unsupervised 
    & \hyperref[sec:electricity-developing]{Ensuring global impact}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & $\bullet$ % transfer
        & % UQ
        & $\bullet$\\% unsupervised 
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{2 \hyperref[sec:transportation]{Transportation}} 
        & % Causal inf
        & % Comp vision
        &% Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:TReducing]{Reducing transport activity}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & $\bullet$% time series
        & % transfer
        & $\bullet$% UQ
        & $\bullet$\\% unsupervised     
   & \hyperref[sec:TEfficient]{Improving vehicle efficiency}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & $\bullet$% rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised    
   & \hyperref[sec:TFuels]{Alternative fuels \& electrification}
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & $\bullet$% rl + control
        & % time series
        & % transfer
        & % UQ
        & $\bullet$ \\% unsupervised    
   & \hyperref[sec:modalshift]{Modal shift}
        & $\bullet$% Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & $\bullet$% time series
        & % transfer
        & $\bullet$% UQ
        & \\% unsupervised    
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{3 \hyperref[sec:buildings-cities]{Buildings and cities}} 
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:indv]{Optimizing buildings}
        & $\bullet$% Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & $\bullet$% rl + control
        & $\bullet$% time series
        & $\bullet$% transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:distr]{Urban planning}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & $\bullet$% time series
        & $\bullet$% transfer
        & % UQ
        & $\bullet$\\% unsupervised 
    & \hyperref[sec:cities]{The future of cities}
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & $\bullet$%% nlp
        & % rl + control
        & %% time series
        & $\bullet$%% transfer
        & $\bullet$% UQ
        & $\bullet$\\% unsupervised 
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{4 \hyperref[sec:industry]{Industry}} 
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:supplychains]{Optimizing supply chains}
        & % Causal inf
        & $\bullet$ %% Comp vision
        & % Interpretable ml
        & % nlp
        & $\bullet$ % rl + control
        & $\bullet$ % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:materialsandconstruction]{Improving materials}
        & %% Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & %% transfer
        & % UQ
        & $\bullet$ \\% unsupervised 
    & \hyperref[sec:demandresponse]{Production \& energy}
        & %% Causal inf
        & $\bullet$%% Comp vision
        & $\bullet$ %% Interpretable ml
        & % nlp
        & $\bullet$% rl + control
        & %% time series
        & %% transfer
        & % UQ
        & \\% unsupervised 
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{5 \hyperref[sec:afolu]{Farms \& forests}} 
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:emissions-detection]{Remote sensing of emissions}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:agriculture]{Precision agriculture}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & $\bullet$% rl + control
        & $\bullet$% time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:peatlands]{Monitoring peatlands}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:forests]{Managing forests}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & $\bullet$ % rl + control
        & $\bullet$ % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{6 \hyperref[sec:ccs]{Carbon dioxide removal}}
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\
    & \hyperref[sec:ccs]{Direct air capture}
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & $\bullet$\\% unsupervised 
    & \hyperref[subsubsec: sequestrativervin]{Sequestering~\cd}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & $\bullet$% UQ
        & $\bullet$\\% unsupervised 
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{7 \hyperref[sec: climate prediction]{Climate prediction}} 
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:climate-models-params]{Uniting data, ML \& climate science}
        & % Causal inf
        & $\bullet$% Comp vision
        & $\bullet$% Interpretable ml
        & % nlp
        & % rl + control
        & $\bullet$% time series
        & % transfer
        & $\bullet$% UQ
        & \\% unsupervised 
    & \hyperref[sec:models-extreme-events]{Forecasting extreme events}
        & % Causal inf
        & $\bullet$% Comp vision
        & $\bullet$% Interpretable ml
        & % nlp
        & % rl + control
        & $\bullet$% time series
        & % transfer
        & $\bullet$% UQ
        & \\% unsupervised 
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{8 \hyperref[sec:societal-impacts]{Societal impacts}} 
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[subsub:ecology]{Ecology}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & $\bullet$% transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[subsub:infrastructure]{Infrastructure}
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & $\bullet$% rl + control
        & $\bullet$% time series
        & % transfer
        & $\bullet$% UQ
        & \\% unsupervised 
    & \hyperref[subsub:social_systems]{Social systems}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & $\bullet$% time series
        & % transfer
        & % UQ
        & $\bullet$\\% unsupervised 
    & \hyperref[subsub:crisis]{Crisis}
        & % Causal inf
        & $\bullet$% Comp vision
        & % Interpretable ml
        & $\bullet$% nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{9 \hyperref[sec:geoengineering]{Solar geoengineering}} 
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[subsub:better-aerosols]{Understanding \& improving aerosols}
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & $\bullet$% time series
        & % transfer
        & $\bullet$% UQ
        & \\% unsupervised 
    & \hyperref[subsub:planetary-control]{Engineering a planetary control system}
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & $\bullet$% rl + control
        & % time series
        & % transfer
        & $\bullet$% UQ
        & \\% unsupervised 
    & \hyperref[subsub:impact-models]{Modeling impacts}
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & $\bullet$% time series
        & % transfer
        & $\bullet$% UQ
        & \\% unsupervised 
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{10 \hyperref[sec:tools-individuals]{Individual action}} 
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:personal_carbon_footprint]{Understanding personal footprint}
        & $\bullet$% Causal inf
        & % Comp vision
        & % Interpretable ml
        & $\bullet$% nlp
        & $\bullet$% rl + control
        & $\bullet$% time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:behavior_change]{Facilitating behavior change}
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & $\bullet$% nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        & $\bullet$\\% unsupervised 
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{11 \hyperref[sec:toolsforsociety]{Collective decisions}} 
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & % rl + control
        & % time series
        & % transfer
        & % UQ
        &  \\% unsupervised 
    & \hyperref[sec:coordination]{Modeling social interactions}
        & % Causal inf
        & % Comp vision
        & $\bullet$ % Interpretable ml
        & % nlp
        & $\bullet$ % rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    & \hyperref[sec:decisionmaking]{Informing policy}
        & $\bullet$ % Causal inf
        & $\bullet$ % Comp vision
        & % Interpretable ml
        & $\bullet$% nlp
        & % rl + control
        & % time series
        & % transfer
        & $\bullet$% UQ
        & $\bullet$\\% unsupervised 
    & \hyperref[subsec:markets]{Designing markets}
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & % nlp
        & $\bullet$% rl + control
        & $\bullet$% time series
        & % transfer
        & % UQ
        & $\bullet$\\% unsupervised 
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{12 \hyperref[sec:education]{Education}} 
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & $\bullet$% nlp
        & $\bullet$% rl + control
        & % time series
        & % transfer
        & % UQ
        & \\% unsupervised 
    \rowcolor{ccai-blue-lightest}
    \multicolumn{2}{l}{13 \hyperref[sec:finance]{Finance}} 
        & % Causal inf
        & % Comp vision
        & % Interpretable ml
        & $\bullet$% nlp
        & % rl + control
        & $\bullet$% time series
        & % transfer
        & $\bullet$% UQ
        & \\% unsupervised 
    \bottomrule
\end{tabular}
\caption{Climate change solution domains, corresponding to sections of this paper, matched with selected areas of ML that are relevant to each. }
\label{tab:summary}
\end{center}
\end{small}
\end{table}


==> figures/old_intro_table.tex <==
\begin{table*}[t]
    \centering
    \begingroup
\renewcommand*{\arraystretch}{1.05}
    \begin{tabular}{l|cccccccccc}
     \toprule 
         & \small{\rotatebox{90}{\parbox{2cm}{Computer \\ vision}}}
         & \small{\rotatebox{90}{NLP}}
         & \small{\rotatebox{90}{\parbox{2cm}{Time-series\\analysis}}}
         & \small{\rotatebox{90}{\parbox{2cm}{Unsupervised\\learning}}}
         & \small{\rotatebox{90}{\parbox{2cm}{RL \&\\Control}}}
        %  & \small{\rotatebox{90}{Robotics}}
         & \small{\rotatebox{90}{\parbox{2cm}{Causal\\inference}}}
         & \small{\rotatebox{90}{\parbox{2cm}{Uncertainty\\quantification}}}
         & \small{\rotatebox{90}{\parbox{2cm}{Transfer\\learning}}}
         & \small{\rotatebox{90}{\parbox{2cm}{Interpretable\\ML}}}
         & \small{\rotatebox{90}{Other}}
     \\ \midrule \\
         \hyperref[sec:electricity-systems]{{\small{Electricity Systems}}}
         &%\ref{sec:electricity-currentSystemImpact},  \ref{sec:electricity-developing}
        \ref{sec:electricity-systems} %\specialcell{\ref{sec:electricity-lowCarbon}\\\ref{sec:electricity-currentSystemImpact}\\ \ref{sec:electricity-developing}}%Computer vision
         & \ref{sec:electricity-lowCarbon}%NLP
         & \specialcell{\ref{sec:electricity-lowCarbon}\\ \ref{sec:electricity-currentSystemImpact}} %Time-series 
         & \ref{sec:electricity-systems}%\specialcell{\ref{sec:electricity-lowCarbon}\\\ref{sec:electricity-currentSystemImpact}\\ \ref{sec:electricity-developing}} %Generative models 
         & \ref{sec:electricity-lowCarbon} %RL \& Control 
        %  & %Robotics 
         & %Causal inference 
         & \specialcell{\ref{sec:electricity-lowCarbon}\\\ref{sec:electricity-currentSystemImpact}} %Uncertainty quantification 
         &%\ref{sec:electricity-lowCarbon}, \ref{sec:electricity-developing}
          \ref{sec:electricity-developing}%Transfer learning 
         & \ref{sec:electricity-lowCarbon} %Interpretable ML 
         & \ref{sec:electricity-lowCarbon} %Other 
     \\ \hline
         \hyperref[sec:transportation]{\small{Transportation}}
         &%\ref{sec:TReducing}, \ref{sec:TEfficient}, \ref{sec:modalshift}
         \specialcell{\ref{sec:TReducing}\\ \ref{sec:TEfficient}\\ \ref{sec:modalshift}}
         %Computer vision
         &%\ref{sec:TReducing}, \ref{sec:modalshift} \specialcell{\ref{sec:TReducing}\\ \ref{sec:modalshift}} %NLP
         & \ref{sec:transportation} %Time-series 
         & \specialcell{\ref{sec:TReducing} \\ \ref{sec:modalshift}} %Generative models 
         & \ref{sec:transportation} %RL \& Control 
        %  & \ref{sec:TEfficient} %Robotics 
         & \specialcell{\ref{sec:TReducing} \\ \ref{sec:modalshift}} %Causal inference 
         & \ref{sec:transportation} %Uncertainty quantification 
         &%\ref{sec:TReducing}, \ref{sec:modalshift}
         \specialcell{\ref{sec:TReducing}\\ \ref{sec:modalshift}}
         %Transfer learning 
         & \ref{sec:transportation} %Interpretable ML 
         & %Other
    \\ \hline
         \hyperref[sec:buildings-cities]{\small{Buildings \& Cities}}
         & \ref{sec:distr} %Computer vision
         & \ref{sec:cities} %NLP
         &\ref{sec:buildings-cities} %\specialcell{\ref{sec:indv}\\ \ref{sec:distr}\\\ref{sec:cities}} %Time-series 
         &\ref{sec:buildings-cities} %\specialcell{\ref{sec:indv}\\ \ref{sec:distr} \\ \ref{sec:cities}} %Generative models 
         & \ref{sec:bldgopt} %RL \& Control 
        %  & %Robotics 
         & \ref{sec:indv} %Causal inference 
         & \ref{sec:cities} %Uncertainty quantification 
         &
         %\ref{sec:distr}, \ref{sec:cities}
       \ref{sec:buildings-cities} %\specialcell{\ref{sec:indv}\\\ref{sec:distr}\\ \ref{sec:cities}} %Transfer learning 
         & %Interpretable ML 
         & %Other
    \\ \hline
         \hyperref[sec:industry]{\small{Industry}}
         & %\ref{sec:supplychains}, \ref{sec:demandresponse}
         \specialcell{\ref{sec:supplychains}\\\ref{sec:demandresponse}} %Computer vision
         & %NLP
         & \ref{sec:demandresponse} %Time-series 
         & \ref{sec:demandresponse} %Generative models 
         &
         %\ref{sec:supplychains}, \ref{sec:materialsandconstruction}, \ref{sec:demandresponse}
        \ref{sec:industry} %\specialcell{\ref{sec:supplychains}\\\ref{sec:materialsandconstruction}\\\ref{sec:demandresponse}} %RL \& Control 
        %  & \ref{sec:demandresponse} %Robotics 
         &
         %\ref{sec:materialsandconstruction}, \ref{sec:demandresponse}
         \specialcell{\ref{sec:materialsandconstruction}\\\ref{sec:demandresponse}} %Causal inference 
         & %Uncertainty quantification 
         &
         %\ref{sec:materialsandconstruction}, \ref{sec:demandresponse}
         \specialcell{\ref{sec:materialsandconstruction}\\\ref{sec:demandresponse}} %Transfer learning 
         & \ref{sec:demandresponse} %Interpretable ML 
         & %Other
    \\ \hline
         \hyperref[sec:afolu]{\small{Farms \& Forests}}
         &
         %\ref{sec:emissions-detection}, \ref{sec:peatlands}, \ref{sec:forests}
         \specialcell{\ref{sec:emissions-detection}\\\ref{sec:peatlands}\\\ref{sec:forests}} %Computer vision
         & %NLP
         & %Time-series 
         & %Generative models 
         & \ref{sec:agriculture} %RL \& Control 
        %  & \ref{sec:agriculture} %Robotics 
         & %Causal inference 
         & %Uncertainty quantification 
         & \ref{sec:forests} %Transfer learning 
         & %Interpretable ML 
         & %Other
    \\ \hline
         \hyperref[sec:ccs]{\small{CO$_2$ Removal}}
         & %Computer vision
         & %NLP
         & \ref{subsubsec: sequestration} %Time-series
         & %Generative models 
         & %RL \& Control 
        %  & %Robotics 
         & %Causal inference 
         & \ref{subsubsec: sequestration} %Uncertainty quantification 
         & \ref{subsubsec: sequestration} %Transfer learning 
         & %Interpretable ML 
         & \ref{subsec:dac} %Other
    \\ \hline
         \hyperref[sec: climate prediction]{\small{Climate Prediction}}
         & \ref{sec: climate models - params} %Computer vision
         & %NLP
         & \ref{sec: climate prediction}
         %\ref{sec: climate models - analysis} %Time-series 
         & %Generative models 
         & %RL \& Control 
        %  & %Robotics 
         & %Causal inference 
         & \ref{sec: climate models - ml+science} %Uncertainty quantification 
         & %Transfer learning 
         & %\ref{sec: climate models - params}, \ref{sec: climate models - ml+science}
         \ref{sec: climate prediction} %Interpretable ML 
         & %Other
    \\ \hline
         \hyperref[sec:societal-impacts]{\small{Societal Impacts}}
         &
         %\ref{subsub:ecology}, \ref{subsub:crisis}
         \specialcell{\ref{subsub:ecology}\\ \ref{subsub:crisis}} %Computer vision
         & \ref{subsub:crisis} %NLP
         &
         %\ref{subsub:infrastructure}, \ref{subsub:social_systems}
         \specialcell{\ref{subsub:infrastructure}\\\ref{subsub:social_systems}} %Time-series 
         & %Generative models 
         & \ref{subsub:infrastructure} %RL \& Control 
        %  & %Robotics 
         & \ref{subsub:social_systems} %Causal inference 
         & \ref{subsub:infrastructure}  % Uncertainty quantification 
         & \ref{subsub:ecology} %Transfer learning 
         & \ref{subsub:social_systems} %Interpretable ML
         & %Other
    \\ \hline
         \hyperref[sec:geoengineering]{\small{Solar Geoengineering}}
         & %Computer vision
         & %NLP
         & \ref{subsub:aerosol-modeling} %Time-series 
         & %Generative models 
         & \ref{subsub:planetary-control} %RL \& Control 
        %  & %Robotics 
         & %Causal inference 
         & %\ref{subsub:aerosol-modeling}, \ref{subsub:planetary-control}
         \specialcell{\ref{subsub:aerosol-modeling}\\\ref{subsub:planetary-control}} %Uncertainty quantification 
         & %Transfer learning 
         & %Interpretable ML 
         & \ref{subsub:better-aerosols} %Other
    \\ \hline
         \hyperref[sec:tools-individuals]{\small{Tools for Individuals}}
         & \ref{sec:personal_carbon_footprint} %Computer vision
         & \ref{sec:personal_carbon_footprint} %NLP
         & \ref{sec:household_energy_impact} %Time-series 
         & \ref{sec:behavior_change}%Generative models 
         & \ref{sec:household_energy_impact} %RL \& Control 
        %  & %Robotics 
         & \ref{sec:personal_carbon_footprint} %Causal inference 
         & %Uncertainty quantification 
         & %Transfer learning 
         & \ref{sec:household_energy_impact} %Interpretable ML 
         & \ref{sec:household_energy_impact} %Other
    \\ \hline
         \hyperref[sec:toolsforsociety]{\small{Tools for Society}}
         & %1 Computer vision
         & \ref{sec:policydesign}  %2 NLP
         &
         \specialcell{\ref{sec:marketsandpricing}\\\ref{sec:policydesign}}%3 Time-series 
         & \ref{sec:multiopt} %4 Generative models 
         & \specialcell{\ref{sec:marketsandpricing}\\ \ref{sec:policydesign}} %5 RL \& Control 
        %  & %Robotics 
         & \specialcell{\ref{sec:policydesign}\\ \ref{sec:multiopt}} %6 Causal inference 
         & \ref{sec:policydesign} %7Uncertainty quantification 
         &\ref{sec:toolsforsociety} %\specialcell{\ref{sec:marketsandpricing}\\ \ref{sec:policydesign}\\ \ref{sec:multiopt}}%8 Transfer learning 
         & \ref{sec:policydesign} %9 Interpretable ML 
         & \specialcell{\ref{sec:policydesign}\\ \ref{sec:multiopt}}%10 Other
    \\ \hline
         \hyperref[sec:education]{\small{Education}}
         & %Computer vision
         & \ref{sec:climate-ed} %NLP
         & %Time-series 
         & %Generative models 
         & \ref{sec:aied}%RL \& Control 
        %  & %Robotics 
         & %Causal inference 
         & %Uncertainty quantification 
         & %Transfer learning 
         & %Interpretable ML 
         & %Other
    \\ \hline
         \hyperref[sec:finance]{\small{Finance}}
         & %Computer vision
         & \ref{sec:climate-analytics}%NLP
         & \ref{sec:finance}
        %  \specialcell{\ref{sec:climate-investment}\\ \ref{sec:climate-analytics}}
         %Time-series 
         & %Generative models 
        %  & %RL \& Control 
         & %Robotics 
         & %Causal inference 
         & \ref{sec:climate-analytics}%Uncertainty quantification 
         & %Transfer learning 
         & %Interpretable ML 
         & %Other
    \\ \bottomrule
    \end{tabular}
    \endgroup
    \caption{Climate change solution domains, along with areas of ML that are relevant to each. Rows of the table correspond to sections of this paper. This table should not be seen as comprehensive.}
    \label{tab:summary}
\end{table*}

